GRAN is superior to GraphRNN: node orderings, kernel- and graph embeddings-based metrics for graph generators

A wide variety of generative models for graphs have been proposed. They are used in drug discovery, road networks, neural architecture search, and program synthesis. Generating graphs has theoretical challenges, such as isomorphic representations -- evaluating how well a generative model performs is difficult. Which model to choose depending on the application domain? We extensively study kernel-based metrics on distributions of graph invariants and manifold-based and kernel-based metrics in graph embedding space. Manifold-based metrics outperform kernel-based metrics in embedding space. We use these metrics to compare GraphRNN and GRAN, two well-known generative models for graphs, and unveil the influence of node orderings. It shows the superiority of GRAN over GraphRNN - further, our proposed adaptation of GraphRNN with a depth-first search ordering is effective for small-sized graphs. A guideline on good practices regarding dataset selection and node feature initialization is provided. Our work is accompanied by open-source code and reproducible experiments.

==> content/broader-impact.tex <==
\section*{Broader Impact}

% TODO
-

%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
%biases in the data. If authors believe this is not applicable to them, authors can simply state this.



==> content/related-work.tex <==
\section{Related Work}\label{sec:related-work}


\paragraph{Graph Generative Models}
While early graph generative model where stochastic, they were not powerful enough to modelize complex depencies found in some real-world networks.
Nowadays, graphs generators using deep learning techniques seek to generate graphs, mimicking given graphs datasets. Several techniques were studied like VAE (\cite{simonovsky2018graphvae,kipf2016variational}) or GAN (\cite{bojchevski2018netgan}). 
The first breaktrough in term of quality and scalabiliy happen with the emergence of autoregressive technique, with the like of GraphRNN (\cite{DBLP:journals/corr/abs-1802-08773}). 
Those methods, due to their sequential nature, needed to restrict the space of studied node ordering in order to make the problem less intractable. 
For exemple, we could use the node ordering given by graph traversals function such as BFS or DFS (DeepGMG by \cite{li2018learning}, DeepGG by \cite{stier2021deepgg}, GraphRNN by \cite{DBLP:journals/corr/abs-1802-08773})

\cite{goyal2020graphgen}
\cite{dai2020scalable}
\cite{obray2021evaluation}



\paragraph{Benchmarking Graph Generators}
Due to the complex and non-euclidean nature of graphs, it is hard to compute any single scalar metrics accounting for similarity. This is why graph statistical (scalar) metrics were first used to measure the performance of graph generative model \cite{bojchevski2018netgan}. 
With GraphRNN, came new metrics based on distance between graph probabilistic distribution using MMD, giving a better picture of some graph properties approximation while working on whole graph datasets. 
First attempts at importing GAN-related metrics such as FID (\cite{heusel2018gans}) were implemented using recent Graph Neural Networks technique such as GIN (\cite{xu2019powerful}), but were only marginally used to give more metrics to work on (\cite{ggmiem,Thompson2020BuildingLU}). 
Concurrently, a study (\cite{anonymous2022on})investigated those newly imported techniques as in our work to put those into a new spotlight, justifying good potential for future use.



==> content/table-GINmesCom.tex <==
\begin{tabular}{llllllll}
            &                & \multicolumn{3}{l}{Community2 (small)}             & \multicolumn{3}{l}{Community2}                    \\ \cline{3-8} 
            &                & FD  $\downarrow $          & F1 PR   $\uparrow $        & F1 DC    $\uparrow $       & FD   $\downarrow $        & F1 PR   $\uparrow $        & F1 DC $\uparrow $          \\ \hline
Re-sampled &                & 6.80           & 0.424           & 0.375           & 1487          & 0.9799          & 1.011           \\ \hline
GRAN       & BFS            & 16.29          & \textbf{0.8207} & 0.3466          & 47782         & 0.8881          & 0.6984          \\
            & DFS            & 26.59          & 0.7951          & \textbf{0.3557} & 21005         & 0.9201          & 0.7523          \\
            & Degree Descent & 31.41          & 0.7335          & 0.2813          & 54148         & 0.8300          & 0.5670          \\
            & Kcore          & 25.18          & 0.7415          & 0.2764          & 22293         & 0.7822          & 0.5559          \\
            & Default        & 74.07          & 0.6491          & 0.2679          & 45217         & 0.8819          & 0.7630          \\ \hline
GraphRNN   & BFS            & 44.69          & 0.2208          & 0.0549          & 12751         & 0.9588          & 0.7883          \\
            & BFS-Max        & 61.37          & 0.2305          & 0.0552          & \textbf{5312} & \textbf{0.9678} & \textbf{0.8590} \\
            & DFS            & \textbf{13.94} & 0.8060          & 0.3336          & 12946         & 0.9242          & 0.7411          \\
            & Uniform        & 182.1          & 0.5762          & 0.1847          & 794711        & 0.1463          & 0.0976          \\ \hline
\end{tabular}


==> content/table-GINmesConcatFull-condensed.tex <==
\begin{table}[tbh]
    \centering
    \begin{tabular}{lllll}
        & \multicolumn{4}{l}{Base dataset configuration} \\
        & ${\boxed\leq^1}$ $\downarrow $        & FD  $\downarrow $           & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
$\ast$   & \textbf{1}       & \textbf{-0.001$\pm$0.001}       & \textbf{1.0$\pm$0.0}    & \textbf{0.994$\pm$0.003} \\ \hline
$\vardiamond$         & 2                & 26639$\pm$14495                 & 0.852$\pm$0.010         & 0.789$\pm$0.016          \\
$\clubsuit$-RNN & 3                & 65917$\pm$24978                 & 0.042$\pm$0.005         & 0.026$\pm$0.006          \\
$\clubsuit$-S   & 4                & 201977$\pm$89750                & 0.0$\pm$0.0             & 0.0$\pm$0.0
\end{tabular}
\begin{tabular}{lllll}
    & \multicolumn{4}{l}{Ladder dataset configuration} \\
    & ${\boxed\leq^1}$ $\downarrow $         & FD  $\downarrow $            & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
$\ast$   & \textbf{1}        & \textbf{-0.002$\pm$0.002}        & \textbf{1.0$\pm$0.0}    & \textbf{0.990$\pm$0.003} \\ \hline
$\vardiamond$         & 2                 & 10228$\pm$11339                  & 0.879$\pm$0.029         & 0.832$\pm$0.069          \\
$\clubsuit$-RNN & 3                 & 91113$\pm$24230                  & 0.047$\pm$0.005         & 0.034$\pm$0.011          \\
$\clubsuit$-S   & 4                 & 212305$\pm$78070                 & 0.003$\pm$0.008         & 0.0006$\pm$0.001        
\end{tabular}
\begin{tabular}{lllll}
    & \multicolumn{4}{l}{Full dataset configuration} \\
    & ${\boxed\leq^1}$ $\downarrow $ & FD  $\downarrow $    & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
$\ast$  & \textbf{1}              & \textbf{-6e-4$\pm$-6e-4} & \textbf{1.0$\pm$0.0}    & \textbf{0.990$\pm$0.007} \\ \hline
$\vardiamond$         & 2                       & 1264$\pm$360             & 0.885$\pm$0.0147        & 0.862$\pm$0.029          \\
$\clubsuit$-RNN & 3                       & 59471$\pm$9750           & 0.048$\pm$0.001         & 0.033$\pm$0.003          \\
$\clubsuit$-S   & 4                       & 91310$\pm$19924          & 0.001$\pm$0.006         & 0.0003$\pm$0.001\\
    \bottomrule
    \multicolumn{5}{l}{$\ast$ Re-Sampled, \small ${\boxed\leq^1}$ Mean Rank}
\end{tabular}
    \caption{
        Concatenation Graph Manifolds metrics on Gr dataset from 10 independently trained GIN.
        All of the metrics show consistent ranking fidelity with the base ranking hypothesis and stability.
        F1 Score metrics are more stable in regards to the dataset configuration, with low variance compared to FD.
    }
    \label{tab:GINmesConcatFull}
\end{table}


==> content/table-GINmesSumFull-condensed.tex <==
\begin{table}[tbh]
    \centering
    \begin{tabular}{lllll}
        & \multicolumn{4}{l}{$\boxed{B}$} \\
        & $\boxed\leq^1$ $\downarrow $   & FD  $\downarrow $  & F1 PR   $\uparrow $ & F1 DC   $\uparrow $ \\ \hline
$\ast$   & 1                         & -0.0010$\pm$0.0007     & 1.0$\pm$0.0             & 0.994$\pm$0.003         \\ \hline
$\vardiamond$         & 2                         & 41004$\pm$14957        & 0.845$\pm$0.006         & 0.79$\pm$0.030          \\
$\clubsuit$-RNN & 3                         & 91512$\pm$24215        & 0.040$\pm$0.010         & 0.019$\pm$0.009         \\
$\clubsuit$-S   & 4                         & 319669$\pm$94417       & 0.0$\pm$0.0             & 0.0$\pm$0.0            
\end{tabular}

    \begin{tabular}{lllll}
        & \multicolumn{4}{l}{$\boxed{L}$} \\
        & $\boxed\leq^1$ $\downarrow $    & FD  $\downarrow $   & F1 PR   $\uparrow $ & F1 DC   $\uparrow $ \\ \hline
$\ast$   & 1                          & -0.0010$\pm$0.0008      & 1.0$\pm$0.0             & 0.992$\pm$0.005         \\ \hline
$\vardiamond$         & 2                          & 30773$\pm$23098         & 0.870$\pm$0.041         & 0.81$\pm$0.10           \\
$\clubsuit$-RNN & 3                          & 127572$\pm$29497        & 0.042$\pm$0.015         & 0.02$\pm$0.01           \\
$\clubsuit$-S   & 4                          & 362265$\pm$149052       & 0.001$\pm$0.006         & 0.003$\pm$0.001        
\end{tabular}

    \begin{tabular}{lllll}
        & \multicolumn{4}{l}{$\boxed{F}$} \\
        & $\boxed\leq^1$ $\downarrow $ & FD  $\downarrow $       & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
$\ast$   & \textbf{1}              & \textbf{-0.0002$\pm$0.0001} & \textbf{1.0$\pm$0.0}    & \textbf{0.990$\pm$0.006} \\ \hline
$\vardiamond$         & 2                       & 737$\pm$340                 & 0.880$\pm$0.016         & 0.847$\pm$0.039          \\
$\clubsuit$-RNN & 3                       & 45270$\pm$16467             & 0.046$\pm$0.006         & 0.027$\pm$0.007          \\
$\clubsuit$-S   & 4                       & 75501$\pm$29895             & 0.0$\pm$0.0             & 0.0$\pm$0.0\\
    \bottomrule
    \multicolumn{5}{l}{\small $\ast$ Re-Sampled, $\boxed\leq^1$ Mean Rank}        
\end{tabular}
    \caption{
        Sum Graph Manifolds metrics on Gr dataset from 10 independently trained GIN.
        All of the metrics show consistent ranking fidelity with the base ranking hypothesis and stability.
        F1 Score metrics are more stable in regards to the dataset configuration, with low variance compared to FD.
    }
    \label{tab:GINmesSumFull}
\end{table}


==> content/table-GINmesWSBA.tex <==
\begin{tabular}{llllllll}
    &                & \multicolumn{3}{l}{Barabasi}                      & \multicolumn{3}{l}{Watts-Stogatz}                \\ \cline{3-8} 
    &                & FD  $\downarrow $          & F1 PR   $\uparrow $        & F1 DC    $\uparrow $       & FD   $\downarrow $        & F1 PR   $\uparrow $        & F1 DC $\uparrow $          \\ \hline
Re-sampled &                & 13.89         & 0.9540          & 0.9567          & 4.450        & 0.9799          & 1.001           \\ \hline
GRAN       & BFS            & \textbf{2399} & \textbf{0.2132} & \textbf{0.0771} & 1332         & 0.4297          & 0.1344          \\
    & DFS            & 3323          & 0.1431          & 0.0315          & 1708         & 0.4546          & 0.2341          \\
    & Degree Descent & 17275         & 0.0366          & 0.0065          & 2189         & 0.2535          & 0.0646          \\
    & Kcore          & 7057          & 0.0514          & 0.0101          & 1843         & 0.2535          & 0.0771          \\
    & Default        & 14364         & 0.0068          & 0.0011          & \textbf{308} & \textbf{0.6964} & \textbf{0.4212} \\ \hline
GraphRNN   & BFS            & 20077         & 0.0             & 0.0             & 44503        & 0.0             & 0.0             \\
    & BFS-Max        & 30684         & 0.0             & 0.0             & 37641        & 0.0             & 0.0             \\
    & DFS            & 9762          & 0.0             & 0.0             & 22886        & 0.0             & 0.0             \\
    & Uniform        & 28248         & 0.0             & 0.0             & 72402        & 0.0             & 0.0             \\ \hline
\end{tabular}


==> content/table-aggr-condensed.tex <==
\begin{tabular}{ll|cc|ccc}
    \toprule
    & & \multicolumn{2}{l}{Grid Generation} & \multicolumn{3}{l}{Perturbation} \\
    \midrule
    & & $\leq^1$ & $\leftrightarrow^2$ & $\leq^1$ & $\leftrightarrow^2$ & $\ostar^3$ \\
    \midrule
    \textbf{FD metric} & $\boxed{B}$ & {\color{Green}$\bm{+}$} & $\uparrow\uparrow$ & {\color{Red}$\bm{-}$} & $\uparrow\uparrow$ &  {\color{Gray}n/a} \\
     & $\boxed{L}$ & {\color{Green}$\bm{+}$} & $\uparrow\uparrow$ & {\color{Red}$\bm{-}$} & $\uparrow\uparrow$ &  {\color{Gray}n/a} \\
     & $\boxed{F}$ & {\color{Green}$\bm{+}$} & $\uparrow$ & {\color{Green}$\bm{+}$} & $\uparrow$ &  {\color{Gray}n/a} \\
    \midrule
    \textbf{F1 metrics} & $\boxed{B}$ & {\color{Green}$\bm{+}$} & $\downarrow$ & {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
    (PRDC) & $\boxed{L}$ & {\color{Green}$\bm{+}$} & $\downarrow$ &  {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
     & $\boxed{F}$ & {\color{Green}$\bm{+}$} & $\downarrow$ &  {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
    \bottomrule
    \multicolumn{7}{l}{\small $\leq^1$ Ranking, $\leftrightarrow^2$ Metric Variance, $\ostar^3$ Sensitivity}
\end{tabular}


==> content/table-aggr.tex <==
\begin{tabular}{ll|cc|ccc}
    \toprule
    & & \multicolumn{2}{l}{Grid Generation} & \multicolumn{3}{l}{Perturbation Comparison} \\
    \midrule
    & & Ranking & Metric Variance & Ranking & Variance & Sensitivity \\
    \midrule
    \textbf{FD metric} & Base Dataset & {\color{Green}$\bm{+}$} & $\uparrow\uparrow$ & {\color{Red}$\bm{-}$} & $\uparrow\uparrow$ &  {\color{Gray}n/a} \\
     & Ladder Dataset & {\color{Green}$\bm{+}$} & $\uparrow\uparrow$ & {\color{Red}$\bm{-}$} & $\uparrow\uparrow$ &  {\color{Gray}n/a} \\
     & Full Dataset & {\color{Green}$\bm{+}$} & $\uparrow$ & {\color{Green}$\bm{+}$} & $\uparrow$ &  {\color{Gray}n/a} \\
    \midrule
    \textbf{F1 metrics} & Base Dataset & {\color{Green}$\bm{+}$} & $\downarrow$ & {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
    (PRDC) & Ladder Dataset & {\color{Green}$\bm{+}$} & $\downarrow$ &  {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
     & Full Dataset & {\color{Green}$\bm{+}$} & $\downarrow$ &  {\color{Gray}n/a} &  {\color{Gray}n/a} & $\uparrow$ \\
    \bottomrule
\end{tabular}


==> content/table-com-condensed.tex <==
\begin{table*}[tbh]
\centering
\begin{tabular}{llllllllll}
\cline{3-10}
           &                & \multicolumn{4}{l}{C2L}                                        & \multicolumn{4}{l}{C2S}                                \\ \cline{3-10} 
           &                & Deg             & Clust           & 4-orbits        & Spec            & Deg             & Clust           & 4-orbits        & Spec            \\ \hline
$\ast$ &                & \textbf{0.0004} & \textbf{0.0036} & \textbf{0.0039} & \textbf{0.0001} & \textbf{0.0005} & \textbf{0.0037} & \textbf{0.0006} & \textbf{0.0011} \\ \hline
E-R        &                & 0.1481          & 0.2562          & 0.1042          & 0.0452          & 0.1715          & 0.1603          & 0.2597          & 0.0730          \\ \hline
$\vardiamond$       & BFS            & 0.0052          & 0.0189          & 0.0070          & 0.0017          & \textbf{0.0009} & 0.0441          & \textbf{0.0074} & 0.0223          \\
           & DFS            & \textbf{0.0012} & 0.0190          & 0.0057          & \textbf{0.0007} & 0.0022          & \textbf{0.0374} & 0.0087          & \textbf{0.0108} \\
           & DegDesc & 0.0262          & 0.0236          & 0.0073          & 0.0029          & 0.0038          & 0.0417          & 0.0138          & 0.0215          \\
           & Kcore          & 0.0082          & 0.0215          & 0.0070          & 0.0011          & 0.0038          & 0.0483          & 0.0405          & 0.0263          \\
           & Default        & 0.0042          & \textbf{0.0115} & \textbf{0.0054} & 0.0010          & 0.0080          & 0.0473          & 0.0801          & 0.0248          \\ \hline
$\clubsuit$   & BFS            & 0.0136          & 0.0400          & \textbf{0.0068} & 0.0092          & 0.0085          & 0.0486          & 0.0088          & 0.0411          \\
           & BFS-Max        & \textbf{0.0075} & \textbf{0.0346} & 0.0075          & \textbf{0.0050} & 0.0041          & \textbf{0.0472} & 0.0103          & 0.0400          \\
           & DFS            & 0.0171          & 0.0524          & 0.0083          & 0.0068          & \textbf{0.0027} & \textbf{0.0472} & \textbf{0.0051} & \textbf{0.0196} \\
           & Uniform        & 0.1594          & 0.2463          & 0.0103          & 0.0079          & 0.0431          & 0.0503          & 1.193           & 0.0478          \\ \hline
\end{tabular}
\caption{
    Ablation study on Node Ordering of GRAN $\vardiamond$ and GraphRNN $\clubsuit$ on C2L and C2S graphs, using reported MMD values.
    Lower values yields better generation quality.
    While on C3L graphs GRAN gets lower MMD values, GraphRNN gets similar results except for the Uniform ordering.
    On C2S graphs both model also gave similar results, with a slight advantage for GRAN.
    GraphRNN-DFS gave comparable results to the other GraphRNN node ordering variants.
}
\label{tab:com}
\end{table*}


==> content/table-node-ordering-wsbacom-condensed.tex <==
\begin{table*}[tbh]
    \centering
    \begin{tabular}{llllllllll}
            &                & \multicolumn{4}{l}{WS}                                         & \multicolumn{4}{l}{BA}                                     \\ \cline{3-10} 
            &                & Deg               & Clust           & 4-orbits          & Spec            & Deg               & Clust           & 4-orbits        & Spec            \\ \hline
    $\ast$ &                & \textbf{2.718e-6} & \textbf{0.0013} & \textbf{9.780e-6} & \textbf{0.0003} & \textbf{3.822e-5} & \textbf{0.0035} & \textbf{0.0047} & \textbf{0.0001} \\ \hline
    E-R        &                & 0.3412            & 1.3495          & 0.1904            & 0.1436          & 0.1074            & 0.6967          & 0.6889          & 0.0564          \\ \hline
    $\vardiamond$       & BFS            & 0.0038            & 0.4425          & 0.0468            & 0.0282          & \textbf{0.0199}   & \textbf{0.0534} & \textbf{0.0360} & 0.0023          \\
            & DFS            & 0.0054            & 0.1818          & 0.0043            & 0.0035          & 0.0339            & 0.0751          & 0.0436          & \textbf{0.0012} \\
            & DegDesc & 0.0180                             & 0.5491                           & 0.0511                             & 0.0090           & 0.0706            & 0.1045          & 0.0553          & 0.0015          \\
            & Kcore          & 0.0208            & 0.4999          & 0.0232            & 0.0091          & 0.0587            & 0.0992          & 0.0379          & 0.0018          \\
            & Default        & \textbf{0.0001}   & \textbf{0.0752} & \textbf{0.0046}   & \textbf{0.0023} & 0.1017            & 0.0967          & 0.0367          & 0.0031          \\ \hline
    $\clubsuit$   & BFS            & 0.0986            & \textbf{0.6891} & 0.1641            & 0.0250          & 0.1083            & \textbf{0.3152} & 0.1525          & 0.0184          \\
            & BFS-Max        & 0.0873            & 0.7388          & 0.2242            & 0.0277          & 0.1280            & 0.3378          & \textbf{0.1377} & 0.0150          \\
            & DFS            & \textbf{0.0780}   & 0.7094          & \textbf{0.1508}   & \textbf{0.0203} & \textbf{0.0342}   & 0.3234          & 0.1690          & \textbf{0.0090} \\
            & Uniform        & 0.1801            & 1.1016          & 1.7263            & 0.0711          & 0.0937            & 0.3775          & 0.1531          & 0.0105          \\

           & & \multicolumn{4}{l}{C2L} & \multicolumn{4}{l}{C2S}  \\
           \hline
$\ast$ &  & \textbf{0.0004} & \textbf{0.0036} & \textbf{0.0039} & \textbf{0.0001} & \textbf{0.0005} & \textbf{0.0037} & \textbf{0.0006} & \textbf{0.0011} \\ \hline
E-R        &                & 0.1481          & 0.2562          & 0.1042          & 0.0452          & 0.1715          & 0.1603          & 0.2597          & 0.0730          \\ \hline
$\vardiamond$       & BFS            & 0.0052          & 0.0189          & 0.0070          & 0.0017          & \textbf{0.0009} & 0.0441          & \textbf{0.0074} & 0.0223          \\
           & DFS            & \textbf{0.0012} & 0.0190          & 0.0057          & \textbf{0.0007} & 0.0022          & \textbf{0.0374} & 0.0087          & \textbf{0.0108} \\
           & DegDesc & 0.0262          & 0.0236          & 0.0073          & 0.0029          & 0.0038          & 0.0417          & 0.0138          & 0.0215          \\
           & Kcore          & 0.0082          & 0.0215          & 0.0070          & 0.0011          & 0.0038          & 0.0483          & 0.0405          & 0.0263          \\
           & Default        & 0.0042          & \textbf{0.0115} & \textbf{0.0054} & 0.0010          & 0.0080          & 0.0473          & 0.0801          & 0.0248          \\ \hline
$\clubsuit$   & BFS            & 0.0136          & 0.0400          & \textbf{0.0068} & 0.0092          & 0.0085          & 0.0486          & 0.0088          & 0.0411          \\
           & BFS-Max        & \textbf{0.0075} & \textbf{0.0346} & 0.0075          & \textbf{0.0050} & 0.0041          & \textbf{0.0472} & 0.0103          & 0.0400          \\
           & DFS            & 0.0171          & 0.0524          & 0.0083          & 0.0068          & \textbf{0.0027} & \textbf{0.0472} & \textbf{0.0051} & \textbf{0.0196} \\
           & Uniform        & 0.1594          & 0.2463          & 0.0103          & 0.0079          & 0.0431          & 0.0503          & 1.193           & 0.0478          \\
    \bottomrule
    \end{tabular}

    \caption{
        Ablation study on the node ordering of GRAN $\vardiamond$ and GraphRNN $\clubsuit$ on BA-, WS-, C2L- and C2S-graphs with MMD values.
        Tiny metric values yields better generation quality.
        Overall GRAN gets lower MMD metric values on both WS and BA datasets, while the choice of node ordering clearly influence results.
        On GraphRNN, DFS ordering give comparable results to the vanilla BFS orderings.
        While on C3L graphs GRAN gets lower MMD values, GraphRNN gets similar results except for the uniform node ordering.
        On C2S graphs both model also gave similar results, with a slight advantage for GRAN.
        GraphRNN-DFS gave comparable results to the other GraphRNN node ordering variants.
    }
    \label{tab:wsba}
    \label{tab:com}
\end{table*}


==> content/table-wsba-condensed.tex <==
\begin{table*}[tbh]
    \centering
    \begin{tabular}{llllllllll}
    \cline{3-10}
            &                & \multicolumn{4}{l}{WS}                                         & \multicolumn{4}{l}{BA}                                     \\ \cline{3-10} 
            &                & Deg               & Clust           & 4-orbits          & Spec            & Deg               & Clust           & 4-orbits        & Spec            \\ \hline
    $\ast$ &                & \textbf{2.718e-6} & \textbf{0.0013} & \textbf{9.780e-6} & \textbf{0.0003} & \textbf{3.822e-5} & \textbf{0.0035} & \textbf{0.0047} & \textbf{0.0001} \\ \hline
    E-R        &                & 0.3412            & 1.3495          & 0.1904            & 0.1436          & 0.1074            & 0.6967          & 0.6889          & 0.0564          \\ \hline
    $\vardiamond$       & BFS            & 0.0038            & 0.4425          & 0.0468            & 0.0282          & \textbf{0.0199}   & \textbf{0.0534} & \textbf{0.0360} & 0.0023          \\
            & DFS            & 0.0054            & 0.1818          & 0.0043            & 0.0035          & 0.0339            & 0.0751          & 0.0436          & \textbf{0.0012} \\
            & DegDesc & 0.0180                             & 0.5491                           & 0.0511                             & 0.0090           & 0.0706            & 0.1045          & 0.0553          & 0.0015          \\
            & Kcore          & 0.0208            & 0.4999          & 0.0232            & 0.0091          & 0.0587            & 0.0992          & 0.0379          & 0.0018          \\
            & Default        & \textbf{0.0001}   & \textbf{0.0752} & \textbf{0.0046}   & \textbf{0.0023} & 0.1017            & 0.0967          & 0.0367          & 0.0031          \\ \hline
    $\clubsuit$   & BFS            & 0.0986            & \textbf{0.6891} & 0.1641            & 0.0250          & 0.1083            & \textbf{0.3152} & 0.1525          & 0.0184          \\
            & BFS-Max        & 0.0873            & 0.7388          & 0.2242            & 0.0277          & 0.1280            & 0.3378          & \textbf{0.1377} & 0.0150          \\
            & DFS            & \textbf{0.0780}   & 0.7094          & \textbf{0.1508}   & \textbf{0.0203} & \textbf{0.0342}   & 0.3234          & 0.1690          & \textbf{0.0090} \\
            & Uniform        & 0.1801            & 1.1016          & 1.7263            & 0.0711          & 0.0937            & 0.3775          & 0.1531          & 0.0105          \\ \hline
    \end{tabular}%
    \caption{
        Ablation study on Node Ordering of GRAN $\vardiamond$ and GraphRNN $\clubsuit$ on BA and WS graphs, using reported MMD values.
        Lower values yields better generation quality.
        Overall GRAN gets lower MMD metrics vazlues on both WS and BA datasets, while the choice of node ordering clearly influence results.
        On GraphRNN, DFS ordering give comparable results to the vanilla BFS orderings.
    }
    \label{tab:wsba}
\end{table*}


==> images/fid_results.tex <==
\chapter{Evaluation using GNN-based metrics}\label{chap:fid_results}

We extend this comparative study by focusing on metrics derived from recent graph neural network techniques. We will use these techniques to see how we need to handle them. First, we will present how we trained the graph neural network (GIN) model. Then we will use the trained model latent space to compute evaluation metrics for generated graphs on some experiments, assessing how well they can rank dissimilarity while varying some training parameters. Finally, we will provide evaluation results from those investigated techniques on the currently trained graph generation models to either confirm or not what was found in the last part using MMD.

\section{Pre-training GNN model in multi-class classification task}
\paragraph{Implementation}
We follow \cite{ggmiem} paper in using GIN \cite{xu2019powerful} as our main Graph classifier technique. We use the implementation of the latter written by the authors of the paper \footnote{https://github.com/weihua916/powerful-gnns}. 
We use the GIN-0 version where we do not train the epsilon coefficient, which we set to 0. For the hyperparameters, we use those advised i.e. 5 layers of GIN with 2 layers of MLP for each, a hidden size of 64, the method of graph pooling and neighborhood pooling are sums. For the pre-training of the models we set the number of epochs to 64, and we use the Adam optimizer with a learning rate of 0.01.

For the used metrics, we use the implemented PRDC pip python library \footnote{https://github.com/clovaai/generative-evaluation-prdc} of the paper \cite{naeem2020reliable} and the Frechet distance implementation from the pytorch-fid git repository \cite{Seitzer2020FID}.

\paragraph{Dataset}
We use the datasets already used in the generation task. We assign a label to each category of graphs. The details on the implementation of datasets will be further explained in the part dealing with the influence of datasets.

\paragraph{Training and classification evaluation}
After training, we quickly evaluate the classification task, which generally works well on this kind of dataset where the graph classes have marked differences. We can see it on the visualization of the t-SNE of the graph embeddings, where the graph embedding clusters are well demarcated.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.70]{trainedfull.png}
    \caption{T-SNE visualization of datasets graphs embeddings, in order ( 0: Watts, 1: Barabasi, 2: Community2 (small),3: Community2,4: ladder,5: grid,6 to 10 : ER baseline graphs)}
    \label{fig:SNE}
\end{figure}
\section{Evaluating graph generators evaluation metrics}
The question of evaluating performance metrics of graph generators has only recently come up. The article evokes criteria for judging comparison metrics, among which we find expressiveness, where the ideal metric would be able to discern samples being more and more distant monotonously.   

To evaluate this aspect, we use two experiments:
\begin{itemize}
    \item We evaluate grid type graphs, one set sampled by the real data distribution (networkx function), and sets from GRAN, GraphRNN and GraphRNN-S \ref{tab:grid} \ref{fig:grid}, models which were trained with their respective recommended hyperparameters (using the DFS ordering for GRAN and BFS from GraphRNN). For the evaluation, we will take for each generator the same amount of graph sample $n=100$ with which we compute the FD and F1 metrics by calculating the embeddings of the latter compared with the same number of real grid graphs being in the dataset. The interest here is that these four sets of graphs correspond to different degrees of fidelity, visually speaking. We expect then that those Graph-embeddings based metrics could rank those models consistently.
    \item We generate graphs from the same data distribution as one of the graphs used in pre-training. We then subject the set of graphs to a perturbation corresponding to an interpolation between this graph and an equivalent random ER graph (like the experience from \cite{DBLP:journals/corr/abs-1802-08773} and \cite{obray2021evaluation}). This is done by randomly perturbing $[0,10,...100\%]$ edges of these graphs by making them rewire with another node of the graph. We thus expect the metrics to react monotonically to those perturbation, thus keeping the similarity rank of each perturbed graph set with the reference set.
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.55]{GridVis[2201].png}
    \caption{Visualisation of generated 2d grid graphs from GRAN, GraphRNN-S and GraphRNN-RNN compared to the training set}
    \label{fig:grid}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{lllll}
    \cline{2-5}
                 & \multicolumn{4}{l}{Grid}            \\ \cline{2-5} 
                 & Deg    & Clust  & 4-orbits & Spec   \\ \hline
    Re-sampled   & 0.0    & 0.0   & 0.0      & 0.0    \\ \hline
    GRAN         & 0.0003 & 0.0004 & 0.0005   & 0.0058 \\ \hline
    GraphRNN-RNN & 0.0047 & 0.0487 & 0.0177   & 0.0213 \\
    GraphRNN-MLP & 0.0627 & 0.0045 & 0.0228   & 0.0292
    \end{tabular}%
    \caption{MMD metrics of 100 sampled graphs compared to the whole base dataset (Resampled mean that we resampled 100 grid graphs from the base data distribution)}
    \label{tab:grid}
    \end{table}

\section{NN-based metrics evaluation using GIN pre-trained on a classification task}

 

\subsection{Pre-training Dataset's influence on NN-based metrics}

In the article \cite{ggmiem}, the dataset was used on the generation tasks, i.e. all the graphs whose topology they wanted to learn and sample from. However, they also added other classes of graphs, notably ladder graphs, while only evaluating grid graphs. They also added bad Ego graphs, graphs sampled from a generation model not sufficiently trained. We do not note any justification, hence the question of the impact of the dataset on these metrics. We want to see if these metrics are sensible to the change of datasets, hence justifying if we need to adjust the dataset to our task.

We take three datasets:
\begin{itemize}
    \item A dataset consisting of all the graphs used for training the graph generators (without enzymes (small) but with grid graphs). We will call it base dataset configuration. (containing 2100 graphs organized in 5 classes, each classes corresponding to one type of graph)
    \item A dataset which is the same as the previous one, but to which we add a new set of graphs in scale (as used by). We will call it ladder dataset. (containing 2600 graphs organized in 6 classes)
    \item A dataset which gathers both these graphs in scale but also ER graphs which are used as reference baseline graph generator (in the GRAN paper \cite{DBLP:journals/corr/abs-1910-00760}) sampling "bad graphs", for each graph G from the same class, an ER graph is created with $|V|=max(|V|_{g},\text{label}(g) = i)$ and parameter $p=\frac{|E|_{g}}{|V|^{2}_{g}}$. We will call it full dataset. (containing 5100 graphs organized in 11 classes)
\end{itemize}

\subsubsection{Experiment 1 : Comparing grid sampled graphs from graph generators}

Using graphs representation from the summation of  graph readouts, we see at first that we do not get fréchet distance values in the same scale in each datasets configuration. While we get such FD metric disparities between datasets configuration, that is not what we get with the F1 PR and F1 DC. We observed that those metric remain relatively stable in regards to the used dataset. We also observe that for each datasets configuration \ref{tab:GINmesSumFull}, we keep the same order between set of graphs.

\begin{table}[h!]
    \centering
    \begin{tabular}{lllll}
        & \multicolumn{2}{l}{Base dataset configuration} &                     &                     \\ \cline{2-5} 
        & Mean Rank $\downarrow $   & FD  $\downarrow $  & F1 PR   $\uparrow $ & F1 DC   $\uparrow $ \\ \hline
Re-sampled   & 1                         & -0.0010±0.0007     & 1.0±0.0             & 0.994±0.003         \\ \hline
GRAN         & 2                         & 41004±14957        & 0.845±0.006         & 0.79±0.030          \\
GraphRNN-RNN & 3                         & 91512±24215        & 0.040±0.010         & 0.019±0.009         \\
GraphRNN-S   & 4                         & 319669±94417       & 0.0±0.0             & 0.0±0.0            
\end{tabular}

    \begin{tabular}{lllll}
        & \multicolumn{2}{l}{Ladder dataset configuration} &                     &                     \\ \cline{2-5} 
        & Mean Rank $\downarrow $    & FD  $\downarrow $   & F1 PR   $\uparrow $ & F1 DC   $\uparrow $ \\ \hline
Re-sampled   & 1                          & -0.0010±0.0008      & 1.0±0.0             & 0.992±0.005         \\ \hline
GRAN         & 2                          & 30773±23098         & 0.870±0.041         & 0.81±0.10           \\
GraphRNN-RNN & 3                          & 127572±29497        & 0.042±0.015         & 0.02±0.01           \\
GraphRNN-S   & 4                          & 362265±149052       & 0.001±0.006         & 0.003±0.001        
\end{tabular}

    \begin{tabular}{lllll}
        & \multicolumn{2}{l}{Full dataset configuration}    &                     &                      \\ \cline{2-5} 
        & Mean Rank $\downarrow $ & FD  $\downarrow $       & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1}              & \textbf{-0.0002±0.0001} & \textbf{1.0±0.0}    & \textbf{0.990±0.006} \\ \hline
GRAN         & 2                       & 737±340                 & 0.880±0.016         & 0.847±0.039          \\
GraphRNN-RNN & 3                       & 45270±16467             & 0.046±0.006         & 0.027±0.007          \\
GraphRNN-S   & 4                       & 75501±29895             & 0.0±0.0             & 0.0±0.0             
\end{tabular}
    \caption{Sum Graph-Embedding metrics on Grid dataset from 10 independently trained GIN}
    \label{tab:GINmesSumFull}
\end{table}

Using graphs representation coming from the concatenation of graph-level redouts at each layer, we found that the ranking of graph generators coming from FD and PRDC metrics remained unchanged through the 10 independents pre-training \ref{tab:GINmesConcatFull}. Having a larger dataset with more classes of graphs reduces the variance on FD through multiple trainings, while PRDC metrics gave consistant results through those three datasets configuration.

\begin{table}[h!]
    \centering
    \begin{tabular}{lllll}
        & \multicolumn{2}{l}{Base dataset configuration} &                     &                      \\ \cline{2-5} 
        & Mean Rank $\downarrow $        & FD  $\downarrow $           & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1}       & \textbf{-0.001±0.001}       & \textbf{1.0±0.0}    & \textbf{0.994±0.003} \\ \hline
GRAN         & 2                & 26639±14495                 & 0.852±0.010         & 0.789±0.016          \\
GraphRNN-RNN & 3                & 65917±24978                 & 0.042±0.005         & 0.026±0.006          \\
GraphRNN-S   & 4                & 201977±89750                & 0.0±0.0             & 0.0±0.0             
\end{tabular}
\begin{tabular}{lllll}
    & \multicolumn{2}{l}{Ladder dataset configuration} &                     &                      \\ \cline{2-5} 
    & Mean Rank $\downarrow $         & FD  $\downarrow $            & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1}        & \textbf{-0.002±0.002}        & \textbf{1.0±0.0}    & \textbf{0.990±0.003} \\ \hline
GRAN         & 2                 & 10228±11339                  & 0.879±0.029         & 0.832±0.069          \\
GraphRNN-RNN & 3                 & 91113±24230                  & 0.047±0.005         & 0.034±0.011          \\
GraphRNN-S   & 4                 & 212305±78070                 & 0.003±0.008         & 0.0006±0.001        
\end{tabular}
\begin{tabular}{lllll}
    & \multicolumn{2}{l}{Full dataset configuration} &                     &                      \\ \cline{2-5} 
    & Mean Rank $\downarrow $ & FD  $\downarrow $    & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1}              & \textbf{-6e-4±-6e-4} & \textbf{1.0±0.0}    & \textbf{0.990±0.007} \\ \hline
GRAN         & 2                       & 1264±360             & 0.885±0.0147        & 0.862±0.029          \\
GraphRNN-RNN & 3                       & 59471±9750           & 0.048±0.001         & 0.033±0.003          \\
GraphRNN-S   & 4                       & 91310±19924          & 0.001±0.006         & 0.0003±0.001        
\end{tabular}
    \caption{Concatenation Graph-Embedding metrics on Grid dataset from 10 independently trained GIN}
    \label{tab:GINmesConcatFull}
\end{table}

\subsubsection{Experiment 2 : Randomly perturbing graphs}

Comparing the experiments performed with the concatenation and summation of the obtained graphs (see figure \ref{FDCONCAT} \ref{FDsum}), we find that with the independently pre-trained model, only the full dataset gives a consistent ranking with FD metric. However, for the other dataset configurations, the FD metric still manages to correctly rank the perturbations up to 60\% ratio where we see FD values decreasing. 

For the F1 PR/DC type metrics, we notice that these scores goes to zero immediately after only 10\% perturbation on grid graphs. Therefore, we could still say that it manages to rank the disturbances correctly but is especially susceptible to this kind of perturbation.

We also extended this experiment by looking at the Watts-Strogatz and Barabasi Albert datasets (see figure \ref{FDconcatBA} \ref{FDconcatWS}), where we saw that the metrics responded monotonically to perturbations, regardless of the choice of the training dataset. Nevertheless, the FD metric's difference gives systematically lower values when computed with the full dataset.

\begin{figure}
    \centering
    \subfloat[Base Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbconcatbase.png}}
    \subfloat[Ladder Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbconcatladder.png}}
    \subfloat[Full Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbconcatfull.png}}\\
    \caption[FD metrics for Grid Graphs, using concatenated graph features]{Plots of FD for perturbed Grid Graph, over 10 indepedents training of GIN, extracting graph feature with concatenation}
    \label{FDCONCAT}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Base Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbsumbase.png}}
    \subfloat[Ladder Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbsumladder.png}}
    \subfloat[Full Dataset]{\includegraphics[width = 0.33\textwidth]{gridperturbsumfull.png}}\\
    \caption[FD metrics for Grid Graphs, using concatenated graph features]{Plots of FD for perturbed Grid Graph, over 10 indepedents training of GIN, extracting graph feature with summation}
    \label{FDsum}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Base Dataset]{\includegraphics[width = 0.33\textwidth]{concatbabaseperturb.png}}
    \subfloat[Full Dataset]{\includegraphics[width = 0.33\textwidth]{concatbafullperturb.png}}\\
    \caption[FD metrics for Barabasi Graphs, using concatenated graph features]{Plots of FD for perturbed Barabasi-Albert Graph, over 10 indepedents training of GIN, extracting graph feature with concatenation}
    \label{FDconcatBA}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Base Dataset]{\includegraphics[width = 0.33\textwidth]{concatwsbaseperturb.png}}
    \subfloat[Full Dataset]{\includegraphics[width = 0.33\textwidth]{concatwsfullperturb.png}}\\
    \caption[FD metrics for Watts Graphs, using concatenated graph features]{Plots of FD for perturbed Watts-Strogatz Graph, over 10 indepedents training of GIN, extracting graph feature with concatenation}
    \label{FDconcatWS}
\end{figure}

\subsection{Impact of node feature initialization}

This question of node feature initialization, asked earlier, is interesting because in this process of making this evaluation practice as generic as possible, using non-informative features or random features can be interesting. We, therefore, want to know if the use of these features negatively impacts the expressiveness of the metrics.

We use the following node features initialization:
\begin{itemize}
    \item The node features initialization used by \cite{ggmiem} in its calculation of the FD, assigns for each node a one-hot-encoding vector corresponding to their node degree. In this case, there would be a problem if we use the same one-hot-encoding on sampled graphs for FD calculation: there is a chance that some node degrees will not be encoded within the one-hot encoding. So, in this case, we map this new node degree to the one-hot encoding of the closest node degree available.
    \item A version where we initialize all the nodes features vector to 1, where we do not distinguish the nodes between them. This approach is more generic since all graphs will have the features of the same nodes. We will call that a constant feature.
    \item We initialize a random integer to the vector, which will be re-generated at each passage in the GIN as in the paper \cite{sato2021random}. This method is also called rGIN.
\end{itemize} 
In the same way as before, we train the model independently ten times according to the different initializations, training them on the so-called full dataset.

We can see \ref{tab:GINmesranda} that for the two approaches consisting in initializing the node features constantly or randomly, the order between GRAN and the versions of GraphRNN is continually respected. However, the order between GraphRNN-RNN and GraphRNN-S is lost compared to the one-hot degree initialization.
   
\begin{table}[h]
\centering
\begin{tabular}{lllll}
    & \multicolumn{4}{l}{With constant feature}                                     \\ \cline{2-5} 
    & Mean Rank  & FD  $\downarrow $   & F1 PR   $\uparrow $ & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1} & \textbf{-8e-5±5e-5} & \textbf{1.0±0.0}    & \textbf{0.975±0.010} \\ \hline
GRAN         & 2          & 211±29              & 0.973±0.015         & 0.973±0.015          \\
GraphRNN-RNN & 4          & 30904±2275          & 0.007±0.010         & 0.052±0.0001         \\
GraphRNN-S   & 3          & 26335±2016          & 0.60±0.027          & 0.056±0.010         
\end{tabular}
\begin{tabular}{lllll}
    & \multicolumn{2}{l}{With random feature (rGIN)} &                      &                      \\ \cline{2-5} 
    & Mean Rank          & FD  $\downarrow $         & F1 PR   $\uparrow $  & F1 DC   $\uparrow $  \\ \hline
Re-sampled   & \textbf{1}         & \textbf{0.87±0.82}        & \textbf{0.988±0.006} & \textbf{1.013±0.021} \\ \hline
GRAN         & 2                  & 61±13                     & 0.967±0.013          & 0.989±0.036          \\
GraphRNN-RNN & 4                  & 8989±1076                 & 0.017±0.006          & 0.058±0.005          \\
GraphRNN-S   & 3                  & 8062±925                  & 0.535±0.074          & 0.065±0.021         
\end{tabular}
\caption{Reported NN-based metrics on Grid dataset on 10 independentely trained GIN (full dataset), using rGIN and constant features}
\label{tab:GINmesranda}
\end{table}

\section{Computing NN-metrics with an untrained GIN}
GIN has been shown to be the most powerful MPNN, it would be interesting to see if it would be possible to use GAN metrics on graph representations from this kind of model. We would then assume that the model is already expressive enough to discriminate between graphs of different types. This is something we already observe when we give the T-SNE visualization of graphs embedding  coming from an untrained model \ref{fig:sneuntrained}.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.70]{untrainedGINSNE.png}
    \caption{T-SNE visualization of datasets graphs embeddings from an untrained GIN, in order ( 0: Watts, 1: Barabasi, 2: Community2 (small),3: Community2,4: ladder,5: grid,6 to 10 : ER baseline graphs)}
    \label{fig:sneuntrained}
\end{figure}

Using the same hyperparameters we will compute graph representations using the untrained GIN. We will initialize node features vectors using degree one-hot-encoding. We will use the one-hot encoding coming from the previous full dataset preparation. We instanciate (initialize weigths) the untrained model 10 times, using the same seed. 

\subsubsection{Experiment : Randomly perturbing graphs}

We evaluate the untrained GIN with the random perturbation experiment with Grid, Watts-Strogatz and Barabasi-Albert graphs. We observe a large variation between instances of the same untrained model, which is mainly due to the fact that the weights are randomly initialized. We can see that either using sum-graph features or concatenation-graph features, FD metrics still reacts monotonically, in a similar way to the measurements collected by the trained models. 
\begin{figure}
    \centering
    \subfloat[Grid]{\includegraphics[width = 0.33\textwidth]{griduntrainedperturbconcat.png}}
    \subfloat[Watts]{\includegraphics[width = 0.33\textwidth]{wattsuntrainedperturbconcat.png}}
    \subfloat[Barabasi]{\includegraphics[width = 0.33\textwidth]{barabasiuntrainedperturbconcat.png}}\\
    \caption[FD metrics for different Graphs on untrained GIN, using concatenated graph features]{Plots of FD for perturbed grpahs, over 10 instance of untrained GIN, extracting graph feature with concatenation}
    \label{FDCONCATUNTRAINED}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Grid]{\includegraphics[width = 0.33\textwidth]{griduntrainedperturbsum.png}}
    \subfloat[Watts]{\includegraphics[width = 0.33\textwidth]{wattsuntrainedperturbsum.png}}
    \subfloat[Barabasi]{\includegraphics[width = 0.33\textwidth]{barabasiuntrainedperturbsum.png}}\\
    \caption[FD metrics for different Graphs on untrained GIN, using sum graph features]{Plots of FD for perturbed grpahs, over 10 instance of untrained GIN, extracting graph feature with summation}
    \label{FDsumUNTRAINED}
\end{figure}

\section{Model-selection with NN-metrics}

Using the models that were periodically saved during the training phases, we want to see if our implementation of the metrics based on a pre-trained GIN model could work. We use here pre-trained models with one-hot encoding feature initialization, trained on the full dataset. We take the example of a GRAN model training on grid graphs on 3000 epochs, where we generate every 300 epochs 100 graphs, that will be then compared to real grid graphs using NN-metrics.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.70]{ImageModelSelection.png}
    \caption{Model selection of GRAN (DFS) training of grid graphs, with plots of FD and F1 (PR/DC) Score , between sampled graphs embeddings and real graph, at several epochs of training}
    \label{fig:modelselect}
\end{figure}

In this example \ref{fig:modelselect}, we see how the model evolves during training. From those charts we can decide for example to select the model trained at 3000th epoch, which showed the best FD and F1 PR Score. This also shows how both FD and F1 Score can be used separately. We see that those metrics gave the same information on the overall performance of this model.

\section{Comparison results between GRAN and GraphRNN}

For the comparison, we train GIN one time on the full dataset configuration using one-hot degree features initialization. Then we use this model to compute all metrics for our comparison study.

We also compute the FD and F1 Score (PR and DC) of synthetic graphs regenerated to provide a lower bound for the FD value and a higher bound for the F1 score.
We notice then directly that it is not the same depending on the dataset. Moreover, in general, the range of FD values varies depending on the dataset, with the lowest values being those in the 2-community (small) dataset. The value of the FD between datasets would then depend on the size and density of the graph. This is not the case for the F1 score, which is always bounded by 1.

Comparing generated graphs, we notice that the GRAN models show lower FD values on the Watts and Barabasi datasets. We note, for example, that the lowest FD value of the generated graph compared to the Watts graphs is that of GRAN with default node ordering, which is consistent with the results collected with the MMD measurements. On the F1 score, we get similar results where GRAN get overall much higher values of F1 PR and F1 DC, while GraphRNN graphs all collected null F1 Scores. This contributes to the argument that GRAN can better capture the data distribution of the graph datasets and thus generate more convincing graphs.

On the 2-Community (small) dataset, the lowest FD and highest F1 Score values are collected on the side of the graphs sampled by GRAN, indicating a better generation quality. Nevertheless, the values remain similar to those of the graphs generated by GraphRNN. 
With GraphRNN, we notice that the DFS node ordering collects a lower FD, while the Uniform node ordering still got the worst score.

On Community2, However, GraphRNN generated graphs collected the better FD and F1 Score (PR-DC). We understand that DFS-GraphRNN graphs collected a worse score than the BFS version (i.e. consistent with human evaluation) but visually, some GRAN and GraphRNN are comparably satisfying. The difference in values may be then a case of lack of diversity more than fidelity.
Still, the Uniform GraphRNN generated graphs got the worse score, which is consistant wuth previous findings.

\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll}
            &                & \multicolumn{3}{l}{Barabasi}                      & \multicolumn{3}{l}{Watts-Stogatz}                \\ \cline{3-8} 
            &                & FD  $\downarrow $          & F1 PR   $\uparrow $        & F1 DC    $\uparrow $       & FD   $\downarrow $        & F1 PR   $\uparrow $        & F1 DC $\uparrow $          \\ \hline
Re-sampled &                & 13.89         & 0.9540          & 0.9567          & 4.450        & 0.9799          & 1.001           \\ \hline
GRAN       & BFS            & \textbf{2399} & \textbf{0.2132} & \textbf{0.0771} & 1332         & 0.4297          & 0.1344          \\
            & DFS            & 3323          & 0.1431          & 0.0315          & 1708         & 0.4546          & 0.2341          \\
            & Degree Descent & 17275         & 0.0366          & 0.0065          & 2189         & 0.2535          & 0.0646          \\
            & Kcore          & 7057          & 0.0514          & 0.0101          & 1843         & 0.2535          & 0.0771          \\
            & Default        & 14364         & 0.0068          & 0.0011          & \textbf{308} & \textbf{0.6964} & \textbf{0.4212} \\ \hline
GraphRNN   & BFS            & 20077         & 0.0             & 0.0             & 44503        & 0.0             & 0.0             \\
            & BFS-Max        & 30684         & 0.0             & 0.0             & 37641        & 0.0             & 0.0             \\
            & DFS            & 9762          & 0.0             & 0.0             & 22886        & 0.0             & 0.0             \\
            & Uniform        & 28248         & 0.0             & 0.0             & 72402        & 0.0             & 0.0             \\ \hline
\end{tabular}%
}
\caption{Reported pretrained GIN-based (with one-hot degree features) metrics on GRAN and GraphRNN for the BA and WS dataset}
\label{tab:GINmesWSBA}
\end{table}

\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llllllll}
                &                & \multicolumn{3}{l}{Community2 (small)}             & \multicolumn{3}{l}{Community2}                    \\ \cline{3-8} 
                &                & FD  $\downarrow $          & F1 PR   $\uparrow $        & F1 DC    $\uparrow $       & FD   $\downarrow $        & F1 PR   $\uparrow $        & F1 DC $\uparrow $          \\ \hline
    Re-sampled &                & 6.80           & 0.424           & 0.375           & 1487          & 0.9799          & 1.011           \\ \hline
    GRAN       & BFS            & 16.29          & \textbf{0.8207} & 0.3466          & 47782         & 0.8881          & 0.6984          \\
                & DFS            & 26.59          & 0.7951          & \textbf{0.3557} & 21005         & 0.9201          & 0.7523          \\
                & Degree Descent & 31.41          & 0.7335          & 0.2813          & 54148         & 0.8300          & 0.5670          \\
                & Kcore          & 25.18          & 0.7415          & 0.2764          & 22293         & 0.7822          & 0.5559          \\
                & Default        & 74.07          & 0.6491          & 0.2679          & 45217         & 0.8819          & 0.7630          \\ \hline
    GraphRNN   & BFS            & 44.69          & 0.2208          & 0.0549          & 12751         & 0.9588          & 0.7883          \\
                & BFS-Max        & 61.37          & 0.2305          & 0.0552          & \textbf{5312} & \textbf{0.9678} & \textbf{0.8590} \\
                & DFS            & \textbf{13.94} & 0.8060          & 0.3336          & 12946         & 0.9242          & 0.7411          \\
                & Uniform        & 182.1          & 0.5762          & 0.1847          & 794711        & 0.1463          & 0.0976          \\ \hline
    \end{tabular}%
    }
    \caption{Reported pretrained GIN-based (with one-hot degree features) metrics on GRAN and GraphRNN for the Community2 (normal and small) graphs}
    \label{tab:GINmesCom}
    \end{table}
